Reduced Label Complexity For Tight $\ell_2$ Regression

Given data ${\rm X}\in\mathbb{R}^{n\times d}$ and labels $\mathbf{y}\in\mathbb{R}^{n}$ the goal is find $\mathbf{w}\in\mathbb{R}^d$ to minimize $\Vert{\rm X}\mathbf{w}-\mathbf{y}\Vert^2$. We give a polynomial algorithm that, \emph{oblivious to $\mathbf{y}$}, throws out $n/(d+\sqrt{n})$ data points and is a $(1+d/n)$-approximation to optimal in expectation. The motivation is tight approximation with reduced label complexity (number of labels revealed). We reduce label complexity by $\Omega(\sqrt{n})$. Open question: Can label complexity be reduced by $\Omega(n)$ with tight $(1+d/n)$-approximation?

==> math.tex <==
\section{Preliminaries}
\label{sec:prelim}

\subsection{\math{\ell_2}-Embeddings}

The matrix \math{\Pi} is an \math{\epsilon}-JLT for an orthogonal matrix
\math{\matU} if
\mld{
  \norm{\matI-\matU\transp\Pi\transp\Pi\matU}_2\le \epsilon.
}
That is, if \math{\Pi\matU} is almost orthogonal. The next lemma summarizes
some of the consequences of an \math{\epsilon}-JLT, which are well known, see
for example
\cite{DMMS07_FastL2_NM10}.
\begin{lemma}\label{lemma:embedding-properties}
Let \math{\matU\in\R^{n,d}} be orthogonal and
\math{\Pi\in\R^{n\times r}}.
Suppose \math{\norm{\matI-\matU\transp\Pi\transp\Pi\matU}\le\epsilon<1}. Then,
\begin{enumerate}
\item \math{|1-\sigma_i^2(\Pi\matU)|\le\epsilon} and
\math{\rank(\Pi\matU)=d}.
\item Let \math{\Pi\matU=\tilde\matU\tilde\Sigma\tilde\matV\transp}.
Then,
\math{\norm{\tilde\Sigma-\tilde\Sigma^{-1}}\le \epsilon/\sqrt{1-\epsilon}}
and \math{\norm{\matI-\tilde\Sigma^{-2}}\le\epsilon/(1-\epsilon)}.
\item
\math{\norm{(\Pi\matU)^{\dagger}-(\Pi\matU)\transp}\le\epsilon/\sqrt{1-\epsilon}}.

\item Let \math{\matA=\matU\Sigma\matV\transp}, where
\math{\Sigma} is positive diagonal and \math{\matV} is orthogonal. Then
\math{(\Pi\matA)^{\dagger}=\matV\Sigma^{-1}(\Pi\matU)^{\dagger}}.
\item \math{\norm{\matI-(\Pi\matU)^{\dagger}(\Pi\matU)^{\dagger\textsc{t}}}\le \epsilon/(1-\epsilon).}
\end{enumerate}
\end{lemma}
\begin{proof}
Part 1 is immediate and implies Part 2 which implies Part 3
because
\math{(\Pi\transp\matU)^{\dagger}=
\tilde\matV\tilde\Sigma^{-1}\tilde\matU\transp}, so
\mand{\norm{(\Pi\transp\matU)^{\dagger}-(\Pi\transp\matU)\transp}
=
\norm{\tilde\matV\tilde\Sigma^{-1}\tilde\matU\transp-\tilde\matV\tilde\Sigma\tilde\matU\transp}
\le
\norm{\tilde\Sigma^{-1}-\tilde\Sigma}.}
Part 4 follows from properties of the pseudo-inveerse. For Part 5, using
\math{\Pi\transp\matU=\tilde\matU\tilde\Sigma\tilde\matV\transp} and
\math{\tilde\matV\tilde\matV\transp=\matI} (since
\math{\Pi\transp\matU} has full rank, so \math{\tilde\matV} is a square
orthogonal matrix),
\mand{\norm{\matI-(\Pi\transp\matU)^{\dagger}(\Pi\transp\matU)^{\dagger\textsc{t}}}
  =
  \norm{\tilde\matV\tilde\matV\transp-\tilde\matV\tilde\Sigma^{-2}\tilde\matV\transp}=\norm{\matI-\Sigma^{-2}}\le\epsilon/(1-\epsilon),}
where the last step follows from Part 2. 
\end{proof}

The next result shows that an \math{\epsilon}-JLT can be used
find a preconditioner.
\begin{lemma}\label{lemma:precond}
  Let \math{\matA=\matU\matSig\matV\transp} be \math{n\times d}, having full rank \math{d}.
  Let \math{\Pi\matA=\matQ\matR}, where \math{\matQ} is any orthogonal
  matrix and \math{\matR} is invertible. 
  Then \math{\sigma_i^2(\matA\matR^{-1})=1/\sigma_{d+1-i}^2(\Pi\matU)}.
\end{lemma}
\begin{proof}
  Consider the SVD of \math{\matA\matR^{-1}
    {\matR^{-1}}\transp\matA\transp}.
  Using
  \math{R^{-1}=(\matQ\transp\Pi\matA)^{-1}=(\Pi\matA)^\dagger\matQ},
  \eqar{
   \matA\matR^{-1}{\matR^{-1}}\transp\matA\transp
   &=&
   \matA(\Pi\matA)^\dagger\matQ\matQ\transp{(\Pi\matA)^\dagger}\transp\matA\transp
   \\
   &=&
   \matU\matSig\matV\transp
   \matV\Sigma^{-1}(\Pi\matU)^{\dagger}
   \matQ\matQ\transp
       {(\Pi\matU)^{\dagger}}\transp\Sigma^{-1}\matV\transp
       \matV\matSig\matU\transp
       \\
       &=&
       \matU(\Pi\matU)^{\dagger}
   \matQ\matQ\transp
       {(\Pi\matU)^{\dagger}}\transp\matU\transp
       \\
       &=&
   \matU(\Pi\matU)^{\dagger}
                  {(\Pi\matU)^{\dagger}}\transp\matU\transp.
                  \label{eq:variational}
   }
  In the last step \math{\matQ\matQ\transp} projects
  onto the column space of \math{\Pi\matU}, hence
  \math{\matQ\matQ\transp
    {(\Pi\matU)^{\dagger}}\transp={(\Pi\matU)^{\dagger}}\transp}.
  Using \math{\Pi\matU=\matU_{\Pi\matU}\matSig_{\Pi\matU}\matV_{\Pi\matU}\transp}, we get
  \math{(\Pi\matU)^{\dagger}
                  {(\Pi\matU)^{\dagger}}\transp=\matV_{\Pi\matU}\matSig_{\Pi\matU}^{-2}\matV_{\Pi\matU}\transp}, hence
  \mld{
    \matA\matR^{-1}{\matR^{-1}}\transp\matA\transp
    =
    \matU\matV_{\Pi\matU}\matSig_{\Pi\matU}^{-2}\matV_{\Pi\matU}\transp
    \matU\transp.
  }
  Since \math{\matU\matV_{\Pi\matU}} is orthogonal, we have
  constructed the SVD of \math{\matA\matR^{-1}{\matR^{-1}}\transp\matA\transp} and so up to a rotation of the row space, we can
  write down the SVD of \math{\matA\matR^{-1}}.
  For some orthogonal \math{d\times d} matrix \math{\matZ},
  \mld{
    \matA\matR^{-1}=
    \matU\matV_{\Pi\matU}\matSig_{\Pi\matU}^{-1}\matZ\transp
  }
  That is, the singular values of
  \math{\matA\matR^{-1}} are the inverses of the singular values of
  \math{\Pi\matU}.
\end{proof}
A useful corollary of Lemma~\ref{lemma:precond}
was observed in \citet{RT08}, namely that
\math{\matA\matR^{-1}} and \math{\Pi\matU} have the same condition
number. Indeed,
\mld{
  \kappa(\matA\matR^{-1})
  =
  \frac{\sigma_1^2(\matA\matR^{-1})}{\sigma_d^2(\matA\matR^{-1})}
  =
  \frac{1/\sigma_d^2(\Pi\matU)}{1/\sigma_1^2(\Pi\matU)}
  =
  \frac{\sigma_1^2(\Pi\matU)}{\sigma_d^2(\Pi\matU)}
  =
  \kappa(\Pi\matU).
}

  
We make heavy use of \math{\epsilon}-JLTs which can be constructed
and applied efficiently.
All constructions use some version of a Johnson-Lindenstrauss Transform.
A finite collection of points can be embeded into lower dimension while
preserving norms to relative error and inner products to additive error.
\begin{lemma}[JLT, \citet{JL1984,Ach03_JRNL}]\label{lemma:JLT}
Let \math{\Pi\in\R^{d\times r}} be a matrix of independent
random signs scaled by
\math{1/\sqrt{r}}.
For \math{n} points \math{\xx_1,\ldots,\xx_n\in
\R^{d}}, let \math{\zz_i=\Pi\transp\xx_i}.
For \math{0<\epsilon<1} and \math{\beta>0}, if
\mld{r\ge\frac{8 +4\beta}{\epsilon^2-2\epsilon^3/3}\ln (n+1),
\label{eq:JLT-r}}
then, with probability at least \math{1-n^{-\beta}},
for all \math{i,j\in[1,n]}:
\eqan{
&(1-\epsilon)\norm{\xx_i-\xx_j}^2\le\norm{\zz_i-\zz_j}^2\le
(1+\epsilon)\norm{\xx_i-\xx_j}^2&\\
&
|\zz_i\transp\zz_j-\xx_i\transp\xx_j|\le
\epsilon(\norm{\xx_i}^2+\norm{\xx_j}^2).
}
\end{lemma}
The \math{\ln(n+1)} comes from adding \math{\bm0} to the points
which preserves all norms. Also, 
\math{\xx_i\transp\xx_j
=\frac12(\norm{\xx_i}^2+\norm{\xx_j}^2-\norm{\xx_i-\xx_j}^2)},
hence inner products are preserved to additive error
\math{\epsilon(\norm{\xx_i}^2+\norm{\xx_j}^2)}.
%

Using this result, we can get \math{\ell_2}-subspace embeddings using a
variety of constructions. The one we will use is an
oblivious fast-Hadamard subspace embedding known as the
Subsampled Random Hadamard Transform (SRHT). A result
from~\citet{T2011} which refines earlier results \cite{earlier} is given
in next lemma which is an  application of Lemmas~3.3 and~3.4 in~\cite{T2011}.
The runtime in the lemma 
is established in~\cite{AL2013}.
\begin{lemma}[{\citet[Lemmas 3.3 and 3.4]{T2011}}]\label{lemma:SRHT-tropp}
  Fix \math{0<\varepsilon\le\frac12}. Let
  \math{\matU\in\R^{n\times d}}
  be orthogonal and \math{\Pi_\textsc{h}\in\R^{r\times n}} an SRHT
  with embedding dimension \math{r}
  satisfying:
  \mld{
    r\ge \frac{12}{5\varepsilon^2}\left(\sqrt{d}+\sqrt{8\ln(3n/\gamma)}\right)^2\ln d
    \ \in\ 
    O\left(\frac{\ln d}{\varepsilon^2}(d+\ln(n/\gamma))\right).
  \label{eq:FJLT-r}}
  Then, with probability at least \math{1-\gamma},
  \math{\Pi_\textsc{h}} is an \math{\epsilon}-JLT for \math{\matU},
  \mld{
    \norm{\matI-\matU\transp\Pi_\textsc{h}\transp\Pi_\textsc{h}\matU}_2\le\varepsilon.
  }
  Further, the product \math{\Pi_\textsc{h}\matA} can be computed in
  time \math{O(nd\ln r)} for any matrix \math{\matA\in\R^{n\times d}}.
\end{lemma}
Note that the SHRT \math{\Pi_{\textsc{h}}} is constructed obliviously of
\math{\matU}. We use the notation \math{\epsilon}-FJLT for such
JLTs that can be applied fast, to distinguish it from the regular
\math{\epsilon}-JLT in Lemma~\ref{lemma:JLT}.

